Data-Driven Goal Recognition in Transhumeral Prostheses Using Process Mining Techniques

A transhumeral prosthesis restores missing anatomical segments below the shoulder, including the hand. Active prostheses utilize real-valued, continuous sensor data to recognize patient target poses, or goals, and proactively move the artificial limb. Previous studies have examined how well the data collected in stationary poses, without considering the time steps, can help discriminate the goals. In this case study paper, we focus on using time series data from surface electromyography electrodes and kinematic sensors to sequentially recognize patients' goals. Our approach involves transforming the data into discrete events and training an existing process mining-based goal recognition system. Results from data collected in a virtual reality setting with ten subjects demonstrate the effectiveness of our proposed goal recognition approach, which achieves significantly better precision and recall than the state-of-the-art machine learning techniques and is less confident when wrong, which is beneficial when approximating smoother movements of prostheses.

==> core.reuse.automata.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reusabe content on automata
%
% First created on: Nov 13, 2021
% Last updated on:  Nov 13, 2021

% Prepared by Artem Polyvyanyy
% Email:    artem.polyvyanyy@gmail.com 
% Homepage: http://polyvyanyy.com
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% core.reuse.automata
% Classical definition of DFA
\begin{ncdefine}{Deterministic Finite Automata}{def:DFAs}{\quad\\}
A \emph{deterministic finite automaton} (DFA) is a tuple $\tuple{Q,\actions,\delta,q_0,A}$, where:
\begin{compactitem}
\item
$Q$ is a finite set of \emph{states};
\item
$\actions$ is a finite set of actions, called the \emph{alphabet};
\item
$\func{\delta}{Q \times \actions}{Q}$ is the \emph{transition function};
\item
$q_0 \in Q$ is the \emph{start state}; and
\item
$A \subseteq Q$ is the set of \emph{accept states}.
\hfill\ensuremath{\lrcorner}
\end{compactitem}
\end{ncdefine}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> core.reuse.ism.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reusabe content for ISMs
%
% First created on: Dec 2, 2019
% Last updated on:  Jan 22, 2019
% Prepared by Artem Polyvyanyy
%
% Email:    artem.polyvyanyy@gmail.com 
% Homepage: http://polyvyanyy.com
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{ncdefine}{Information model}{def:info:model}{\quad\\}
An \emph{information model} is a 5-tuple $(E,R,\rho,\eta,\Psi)$, where:
\begin{compactitem}
\item
$E \subseteq \powerset{\identifiers}$ is a finite set of \emph{entity types};
\item
$R \subseteq \labels$ is a finite set of \emph{relation types};
\item
$\func{\rho}{R}{\kleenestar{E}}$ is a \emph{relation definition function} that maps every relation type onto a finite sequence of entity types;
\item
$\func{\eta}{E}{R}$ is an \emph{entity relation definition function} that maps every entity type onto a relation type such that
$\eta$ is injective and for every $e \in E$ it holds that $\funcCall{\rho}{\funcCall{\eta}{e}}=\sequence{e}$, $\funcCall{\eta}{e}$ is called the \emph{entity relation} of $e$;
\item
$\Psi$ is a collection of statements in first-order logic that for every $r \in R$, $n=|\funcCall{\rho}{r}|$, 
(i) can use predicate $r$ over the domain $\identifiers^n$, called the \emph{relation predicate} of $r$, 
and (ii) contains the statement:
\[
\mathop{\bigforall} i \in \identifiers^n \holds \left(\funcCall{r}{i(1),\ldots,i(n)} \implies \left(\bigwedge_{k=1}^{n} \funcCall{\funcCall{\eta}{\funcCall{\rho}{r}(k)}}{i(k)}\right)\right),
\]
%\[ deprecated formulation
%\mathop{\bigforall}_{j=1}^{n} i_j \in \identifiers \holds \left(\funcCall{r}{i_1,\ldots,i_n} \implies \left(\bigwedge_{k=1}^{n} \funcCall{\funcCall{\eta}{\funcCall{\rho}{r}(k)}}{i_k}\right)\right),
%\]
called the \emph{relation predicate statement} of $r$.
\hfill\ensuremath{\lrcorner}
\end{compactitem}	
\end{ncdefine}

\begin{define}{Population, Fact}{def:info:model:population}{\quad\\}
A \emph{population} of an information model $(E,R,\rho,\eta,\Psi)$ is a function $\func{\pi}{R}{\powerset{\bigcup_{n \in \natnum}{\identifiers^n}}}$
such that every element in the population is correctly typed, \ie
for every $r \in R$ it holds that $\funcCall{\pi}{r} \in \powerset{\prod_{i=1}^{|\funcCall{\rho}{r}|}{\!\funcCall{\rho}{r}(i)}}$.
An element in $\funcCall{\pi}{r}$ is called a \emph{fact}.
\end{define}

==> core.reuse.petri.tex <==
A Petri net is a model of a distributed system~\cite{Reisig98}.

\begin{define}{Petri net}{def:petri:net}{\quad\\}
A \emph{(labeled) Petri net}, or a \emph{net}, $N$ is a quintuple $\tuple{P,T,F,\Lambda,\lambda}$, where
$P$ is a finite set of \emph{places},
$T$ is a finite set of \emph{transitions},
$F \subseteq (P \times T) \cup (T \times P)$ is the \emph{flow relation},
$\Lambda$ is a set of \emph{labels}, such that $\tau \in \Lambda$ is the \emph{silent label} and sets $P$, $T$, and $\Lambda$ are pairwise disjoint, and 
$\func{\lambda}{T}{\Lambda}$ is the \emph{labeling function}.
\end{define}

\noindent
If $\funcCall{\lambda}{t}=\tau$, $t \in T$, then $t$ is \emph{silent}; otherwise $t$ is \emph{observable}.
Observable transitions represent activities from the problem domain, whereas silent transitions encode internal actions of the system. 
A \emph{marking} of a net encodes its state.

\begin{define}{Marking}{def:marking}{\quad\\}
A \emph{marking} $M$ of a net $\tuple{P,T,F,\Lambda,\lambda}$ is a multiset over places $P$.
\end{define}

\noindent
A net system is a net with an initial and final markings.

\begin{define}{Net system}{def:net:system}{\quad\\}
A \emph{net system}, or a \emph{system}, $S$ is a triple $\tuple{N,M_{\mathit{ini}},M_{\mathit{fin}}}$, where 
$N=\tuple{P,T,F,\Lambda,\lambda}$ is a net,
$M_{\mathit{ini}}$ is the \emph{initial marking} of $N$, and 
$M_{\mathit{fin}}$ is the \emph{final marking} of $N$.
\end{define}

\noindent
Let $N=\tuple{P,T,F,\Lambda,\lambda}$ be a net.
A transition $t \in T$ is \emph{enabled} in a marking $M$ of $N$, denoted by $\enabled{N}{M}{t}$, if every \emph{input place} of $t$ contains at least one token, \ie 
$\predicate{\forall}{p \in \setbuilder{x \in P}{(x,t) \in F}}{\funcCall{M}{p} > 0}$. 
An enabled transition $t \in T$ can \emph{occur}.
An occurrence of $t$ \emph{leads to} a fresh marking $M' = (M \setminus \setbuilder{x \in P}{(x,t) \in F}) \uplus \setbuilder{y \in P}{(t,y) \in F}$ of $N$, denoted by $\occurrence{N}{M}{t}{M'}$.

A finite sequence of transitions $\sigma=\sequence{t_1,t_2,\ldots,t_n} \in \kleenestar{T}$, $n \in \natnumwithzero$, is an \emph{occurrence sequence} of a net $N$ at marking $M$, if $\sigma$ is empty or there exists a sequence of markings $\sequence{M_0,M_1,\ldots,M_n}$, such that $M_0=M$ and for every position $i \in \intintervalcc{1}{n}$ in $\sigma$ it holds that $\occurrence{N}{M_{i-1}}{t_i}{M_i}$.
We say that $\sigma$ \emph{leads $N$ from $M$ to $M_n$} and denote this fact by $\leadsfromto{N}{M}{\sigma}{M_n}$.
Finally, $\sigma$ is an \emph{execution} of a net system $\tuple{N,M_\mathit{ini},M_\mathit{fin}}$ if $\sigma$ leads $N$ from $M_\mathit{ini}$ to $M_\mathit{fin}$.

==> fig/tikz/pn1.tex <==
\begin{tikzpicture}[thick,font=\Large]

    \node[draw,align=center,circle,minimum size=1cm] (n1) at (1.5,-9.0) {net source};
    \node[draw,align=center,circle,minimum size=1cm] (n2) at (16.5,-5.5) {net sink};
    \node[draw,align=center,circle,minimum size=1cm] (n3) at (9.0,-10.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n4) at (12.5,-3.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n5) at (16.5,-2.0) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n6) at (12.5,-10.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n7) at (5.0,-9.0) {p};
    
    \node[draw,align=center,minimum size=1cm] (n8) at (10.5,-3.5) {};
    \node at (n8.center) {4};
    \node[draw,align=center,minimum size=1cm] (n9) at (10.5,-10.5) {};
    \node at (n9.center) {1};
    \node[draw,align=center,minimum size=1cm] (n10) at (14.5,-7.0) {};
    \node at (n10.center) {7};
    \node[draw,align=center,minimum size=1cm] (n21) at (7.0,-14.0) {};
    \node at (n21.center) {8 -> end};
    \node[draw,align=center,minimum size=1cm] (n20) at (3.0,-9.0) {};
    \node at (n20.center) {8};
    \node[draw,align=center,minimum size=1cm] (n12) at (14.5,-2.0) {};
    \node at (n12.center) {2};
    \node[draw,align=center,minimum size=1cm] (n11) at (14.5,-5.5) {};
    \node at (n11.center) {4};
    \node[draw,align=center,minimum size=1cm] (n22) at (14.5,-12.5) {};
    \node at (n22.center) {1 -> end};
    \node[draw,align=center,minimum size=1cm] (n14) at (18.0,-2.0) {};
    \node at (n14.center) {4};
    \node[draw,align=center,minimum size=1cm] (n13) at (18.0,-3.5) {};
    \node at (n13.center) {7};
    \node[draw,align=center,minimum size=1cm] (n16) at (14.5,-9.0) {};
    \node at (n16.center) {8};
    \node[draw,align=center,minimum size=1cm] (n15) at (14.5,-10.5) {};
    \node at (n15.center) {2};
    \node[draw,align=center,minimum size=1cm] (n18) at (7.0,-12.5) {};
    \node at (n18.center) {1};
    \node[draw,align=center,minimum size=1cm] (n17) at (7.0,-10.5) {};
    \node at (n17.center) {7};
    \node[draw,align=center,minimum size=1cm] (n19) at (7.0,-2.0) {};
    \node at (n19.center) {8};
    
    \draw[-{Latex[length=3mm]}] (n3) -- (n8);
    \draw[-{Latex[length=3mm]}] (n15) -- (n5);
    \draw[-{Latex[length=3mm]}] (n9) -- (n6);
    \draw[-{Latex[length=3mm]}] (n19) -- (n7);
    \draw[-{Latex[length=3mm]}] (n7) -- (n17);
    \draw[-{Latex[length=3mm]}] (n7) -- (n18);
    \draw[-{Latex[length=3mm]}] (n4) -- (n12);
    \draw[-{Latex[length=3mm]}] (n6) -- (n15);
    \draw[-{Latex[length=3mm]}] (n3) -- (n9);
    \draw[-{Latex[length=3mm]}] (n16) -- (n7);
    \draw[-{Latex[length=3mm]}] (n18) -- (10.5,-13.0) -- (n6);
    \draw[-{Latex[length=3mm]}] (n6) -- (n16);
    \draw[-{Latex[length=3mm]}] (n13) -- (16.5,-7.5) -- (14.5,-16.5) -- (10.5,-16.5) -- (n3);
    \draw[-{Latex[length=3mm]}] (n7) -- (n21);
    \draw[-{Latex[length=3mm]}] (n8) -- (n4);
    \draw[-{Latex[length=3mm]}] (n12) -- (n5);
    \draw[-{Latex[length=3mm]}] (n17) -- (n3);
    \draw[-{Latex[length=3mm]}] (n6) -- (n22);
    \draw[-{Latex[length=3mm]}] (n4) -- (n10);
    \draw[-{Latex[length=3mm]}] (n1) -- (n20);
    \draw[-{Latex[length=3mm]}] (n7) -- (n19);
    \draw[-{Latex[length=3mm]}] (n4) -- (n11);
    \draw[-{Latex[length=3mm]}] (n11) -- (n4);
    \draw[-{Latex[length=3mm]}] (n20) -- (n7);
    \draw[-{Latex[length=3mm]}] (n14) -- (16.5,-4.0) -- (n4);
    \draw[-{Latex[length=3mm]}] (n22) -- (n2);
    \draw[-{Latex[length=3mm]}] (n5) -- (n14);
    \draw[-{Latex[length=3mm]}] (n21) -- (14.5,-14.5) -- (n2);
    \draw[-{Latex[length=3mm]}] (n10) -- (10.5,-7.5) -- (n3);
    \draw[-{Latex[length=3mm]}] (n5) -- (n13);
    
    \end{tikzpicture}

==> fig/tikz/pn2.tex <==
\begin{tikzpicture}[thick,font=\Large]

    \node[draw,align=center,circle,minimum size=1cm] (n1) at (1.5,-3.5) {net source};
    \node[draw,align=center,circle,minimum size=1cm] (n2) at (31.5,-2.0) {net sink};
    \node[draw,align=center,circle,minimum size=1cm] (n3) at (20.0,-7.0) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n4) at (9.0,-3.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n5) at (27.5,-2.0) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n6) at (24.0,-2.0) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n7) at (20.0,-3.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n8) at (16.5,-3.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n9) at (12.5,-3.5) {p};
    \node[draw,align=center,circle,minimum size=1cm] (n10) at (5.0,-5.5) {p};
    
    \node[draw,align=center,minimum size=1cm] (n12) at (22.0,-9.0) {};
    \node at (n12.center) {5};
    \node[draw,align=center,minimum size=1cm] (n11) at (22.0,-7.0) {};
    \node at (n11.center) {3};
    \node[draw,align=center,minimum size=1cm] (n14) at (29.5,-3.5) {};
    \node at (n14.center) {6};
    \node[draw,align=center,minimum size=1cm] (n13) at (10.5,-3.5) {};
    \node at (n13.center) {7};
    \node[draw,align=center,minimum size=1cm] (n16) at (22.0,-3.5) {};
    \node at (n16.center) {9};
    \node[draw,align=center,minimum size=1cm] (n15) at (25.5,-2.0) {};
    \node at (n15.center) {6};
    \node[draw,align=center,minimum size=1cm] (n18) at (18.0,-7.0) {};
    \node at (n18.center) {3};
    \node[draw,align=center,minimum size=1cm] (n17) at (22.0,-5.5) {};
    \node at (n17.center) {0};
    \node[draw,align=center,minimum size=1cm] (n19) at (18.0,-2.0) {};
    \node at (n19.center) {5};
    \node[draw,align=center,minimum size=1cm] (n21) at (14.5,-3.5) {};
    \node at (n21.center) {0};
    \node[draw,align=center,minimum size=1cm] (n20) at (18.0,-3.5) {};
    \node at (n20.center) {9};
    \node[draw,align=center,minimum size=1cm] (n23) at (7.0,-7.0) {};
    \node at (n23.center) {7};
    \node[draw,align=center,minimum size=1cm] (n22) at (7.0,-5.5) {};
    \node at (n22.center) {1};
    \node[draw,align=center,minimum size=1cm] (n25) at (3.0,-3.5) {};
    \node at (n25.center) {1};
    \node[draw,align=center,minimum size=1cm] (n24) at (3.0,-5.5) {};
    \node at (n24.center) {8};
    \node[draw,align=center,minimum size=1cm] (n26) at (29.5,-2.0) {};
    \node at (n26.center) {6 -> end};
    
    \draw[-{Latex[length=3mm]}] (n17) -- (18.0,-6.0) -- (n8);
    \draw[-{Latex[length=3mm]}] (n8) -- (n20);
    \draw[-{Latex[length=3mm]}] (n10) -- (n22);
    \draw[-{Latex[length=3mm]}] (n26) -- (n2);
    \draw[-{Latex[length=3mm]}] (n24) -- (n10);
    \draw[-{Latex[length=3mm]}] (n11) -- (n3);
    \draw[-{Latex[length=3mm]}] (n19) -- (n6);
    \draw[-{Latex[length=3mm]}] (n18) -- (n3);
    \draw[-{Latex[length=3mm]}] (n14) -- (n5);
    \draw[-{Latex[length=3mm]}] (n15) -- (n5);
    \draw[-{Latex[length=3mm]}] (n7) -- (n16);
    \draw[-{Latex[length=3mm]}] (n8) -- (n18);
    \draw[-{Latex[length=3mm]}] (n16) -- (n7);
    \draw[-{Latex[length=3mm]}] (n23) -- (9.0,-6.0) -- (10.5,-6.0) -- (n9);
    \draw[-{Latex[length=3mm]}] (n20) -- (n7);
    \draw[-{Latex[length=3mm]}] (n3) -- (n12);
    \draw[-{Latex[length=3mm]}] (n5) -- (n14);
    \draw[-{Latex[length=3mm]}] (n13) -- (n9);
    \draw[-{Latex[length=3mm]}] (n1) -- (n25);
    \draw[-{Latex[length=3mm]}] (n22) -- (n4);
    \draw[-{Latex[length=3mm]}] (n7) -- (n17);
    \draw[-{Latex[length=3mm]}] (n21) -- (n8);
    \draw[-{Latex[length=3mm]}] (n8) -- (n19);
    \draw[-{Latex[length=3mm]}] (n5) -- (n26);
    \draw[-{Latex[length=3mm]}] (n12) -- (n6);
    \draw[-{Latex[length=3mm]}] (n6) -- (n15);
    \draw[-{Latex[length=3mm]}] (n25) -- (n4);
    \draw[-{Latex[length=3mm]}] (n1) -- (n24);
    \draw[-{Latex[length=3mm]}] (n9) -- (n21);
    \draw[-{Latex[length=3mm]}] (n4) -- (n13);
    \draw[-{Latex[length=3mm]}] (n3) -- (n11);
    \draw[-{Latex[length=3mm]}] (n10) -- (n23);
    
    \end{tikzpicture}

==> fig/tpl/Petri_nets.tex <==
\begin{figure}[h!]
\begin{center}
\vspace{-3mm}
\begin{tikzpicture}[scale=0.65, transform shape, ->, >=stealth', shorten >=1pt, auto, node distance=20mm, on grid, semithick, transition/.style={fill=red!10, draw, minimum size=9mm, drop shadow}, place/.style={fill=blue!10, draw, circle, minimum size=9mm, drop shadow}]

\node[place,label=90:\large $p_0$]				(p0) 											{\Large $\bullet$};
\node[transition,label=90:\large $t_0$]		(t0) [right=of p0] 				{\Large $\texttt{a}$};
\node[place,label=90:\large $p1$] 				(p1) [above right=of t0]	{};
\node[place,label=270:\large $p_2$] 			(p2) [below right=of t0]	{};
\node[transition,label=90:\large $t_1$] 	(t1) [right=of p1]				{\Large $\texttt{b}$};
\node[transition,label=270:\large $t_3$] 	(t3) [right=of p2]				{\Large $\texttt{c}$};
\node[transition,label=0:\large $t_2$] 		(t2) [below right=of p1,xshift=17pt]				{\Large $\texttt{d}$};
\node[place,label=90:\large $p3$] 				(p3) [right=of t1]				{};
\node[place,label=270:\large $p4$] 				(p4) [right=of t3]				{};
\node[transition,label=90:\large $t_4$] 	(t4) [below right=of p3]	{\Large $\texttt{e}$};
\node[place,label=90:\large $p5$] 				(p5) [right=of t4]				{};

\path (p0) edge node {} (t0)
			(t0) edge node {} (p1)
					 edge node {} (p2)
			(p1) edge node {} (t1)
			(p2) edge node {} (t3)
			(t1) edge node {} (p3)
			(t3) edge node {} (p4)
			(t2) edge node {} (p1)
					 edge node {} (p2)
			(p3) edge node {} (t2)
					 edge node {} (t4)
			(p4) edge node {} (t2)
					 edge node {} (t4)
			(t4) edge node {} (p5)
;
\end{tikzpicture}
\vspace{-2mm}
\caption{A Petri net.}
\label{fig:petri:net}
\vspace{-2mm}
\end{center}
\end{figure}

==> fig/tpl/automata.tex <==
\begin{figure}[h!]
\begin{center}
\vspace{-5mm}
\begin{tikzpicture}[scale=0.65, transform shape, ->, >=stealth', shorten >=1pt, auto, initial text=, node distance=20mm, on grid, semithick, every state/.style={fill=orange!20, draw, circular drop shadow, text=black, minimum size=9mm}]
\node[initial,state,label=270:$s_0$]	(s0) 											{$0$};
\node[state,label=270:$s_1$]					(s1) [right=of s0] 				{$0$};
\node[state,label=0:$s_2$]						(s2) [above right=of s1]	{$0$};
\node[state,label=270:$s_3$] 					(s3) [below right=of s2]	{$0$};
\node[state,label=0:$s_4$] 					  (s4) [below right=of s1]	{$\nicefrac{1}{5}$};
\node[state,label=270:$s_5$] 				  (s5) [right=of s3]				{$1$};

\path (s0) edge node {$\texttt{a}(1)$} (s1)
			(s1) edge node {$\texttt{b}(\nicefrac{1}{2})$} (s2)
			     edge node[below, xshift=-14pt, yshift=-2pt] {$\texttt{c}(\nicefrac{1}{2})$} (s4)
			(s2) edge node {$\texttt{c}(1)$} (s3)
			(s3) edge node[above]  {$\texttt{d}(\nicefrac{1}{2})$} (s1)
					 edge node {$\texttt{e}(\nicefrac{1}{2})$} (s5)
			(s4) edge node[below, xshift=16pt, yshift=-2pt] {$\texttt{b}(\nicefrac{4}{5})$} (s3);
\end{tikzpicture}
\vspace{-2mm}
\caption{An SDFA.}
\label{fig:SDFA}
\vspace{-4mm}
\end{center}
\end{figure}

==> tables/t_test.tex <==
\begin{table}[ht!]
    \centering
    \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{|c|cc|cc|c|}
        \hline
             & \multicolumn{2}{c|}{PM} & \multicolumn{2}{c|}{LSTM} & LDA \\ \cline{2-6} 
             & p          & r          & p           & r           &     \\ \hline
        PM   &            &            &             &             &     \\ \hline
        LSTM & 1.185e-03  & 4.173e-34  &             &             &     \\ \hline
        LDA  & 5.153e-10  & 1.188e-34  & 3.272e-07   & 3.272e-07   &     \\ \hline
        \end{tabular}%
    }
    \caption{The p-values of pairwise t-tests between the three approaches on precision (P) and recall (r).}
    \label{tab:t-test}
\end{table}


% \begin{table}[ht!]
%     \centering
%     \resizebox{0.3\textwidth}{!}{%
%     \begin{tabular}{cccc}
%         & PM        & LSTM      & LDA \\
%     PM   &           &           &     \\
%     LSTM & 1.185e-03 &           &     \\
%     LDA  & 5.153e-10 & 3.272e-07 &    
%     \end{tabular}%
%     }
%     \caption{P-values (precision)}
%     \label{tab:p_p_values}
% \end{table}

% \begin{table}[ht!]
%     \centering
%     \resizebox{0.3\textwidth}{!}{%
%     \begin{tabular}{cccc}
%         & PM        & LSTM      & LDA \\
%     PM   &           &           &     \\
%     LSTM & 4.173e-34 &           &     \\
%     LDA  & 1.188e-34 & 3.272e-07 &    
%     \end{tabular}%
%     }
%     \caption{P-values (recall)}
%     \label{tab:r_p_values}
% \end{table}

==> tpl/icpm/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

